Near-field 6G Networks: Why Mobile Terahertz Communications MUST Operate in the Near Field

Near-field mobile terahertz (THz) communications is one of the candidate enablers for high-rate wireless data exchange in sixth-generation (6G) networks. However, operating in the THz near field brings both attractive opportunities and severe challenges. Hence, it becomes of interest to explore if it is possible to design a realistic mobile THz communication system without working in the THz near field. To answer this question, a mathematical framework is presented modeling a mobile THz link that works exclusively in the far field. The study leads to an interesting theoretical conclusion: while the actual frequency is of (almost) no interest, such a system must operate over a limited bandwidth not exceeding a certain threshold. It is then numerically shown that operating only in the far field imposes stringent limitations on mobile THz communications, thus making them less attractive to prospective high-rate services. In contrast, it is shown that a stationary THz link can still be broadband even when staying exclusively in the THz far field. Hence, broadband mobile THz communications MUST be near-field, while broadband stationary THz links do not have to.

==> OLD/mobile_thz_math_backup.tex <==
% ----------------------------------------------------------------------------
% Citation database
% ----------------------------------------------------------------------------

@STRING{ASPDAC = "Proceedings of the Asia and South Pacific Design Automation Conference (ASPDAC)"}
@STRING{DAC = "Proceedings of the Design Automation Conference (DAC)"}
@STRING{DATE = "Proceedings of the Design, Automation and Test in Europe (DATE) Conference"}
@STRING{CODES = "Proceedings of the International Symposium on Hardware-Software Codesign (CODES)"}
@STRING{EDAC = "Proceedings of the European Design Automation Conference (Euro-DAC)"}
@STRING{EDTC = "Proceedings of the European Design and Test Conference"}
@STRING{ICCD = "Proceedings of the International Conference on Computer Design (ICCD)"}
@STRING{ICCAD = "Proceedings of the International Conference on Computer Aided Design (ICCAD)"}
@STRING{ISSS = "Proceedings of the International Symposium on System Synthesis"}
@STRING{SASIMI = "Proceedings of the Workshop of Synthesis and System Integration of Mixed Information Technologies"}
@STRING{ESC = "Proceedings of the Embedded System Conference (ESC)"}
@STRING{TCAD = "IEEE Transactions on Computer-Aided Design of Intergrated Circuits and Systems (TCAD)"}
@STRING{TCOMP = "IEEE Transactions on Computers"}
@STRING{TSP = "IEEE Transactions on Signal Processing"}
@STRING{TVLSI = "IEEE Transactions on VLSI Systems"}
@STRING{TPDS = "IEEE Transactions on Parallel and Distributed Systems"}
@STRING{D&T = "IEEE Design and Test of Computers"}
@STRING{JACM = "Journal of the ACM"}
@STRING{TODAES = "ACM Transactions on Design Automation of Electronic Systems"}
@STRING{Kluwer = "Kluwer Academic Publishers"}
@STRING{Prentice = "Prentice Hall"}

@STRING{ICS = "Information and Computer Science"}
@STRING{UCI = "University of California, Irvine"}
@STRING{CECS = "Center for Embedded Computer Systems"}


@INPROCEEDINGS{petrov_infocom,
  author={Petrov, Vitaly and Moltchanov, Dmitri and Jornet, Josep Miquel and Koucheryavy, Yevgeni},
  booktitle={Proc. of the IEEE Conference on Computer Communications Workshops (INFOCOM WKSHPS)}, 
  title={Exploiting Multipath Terahertz Communications for Physical Layer Security in Beyond {5G} Networks}, 
  year={2019},
  pages={865-872},
  month = {April},
  }


@ARTICLE{near_field_6G_magazine,
  author={Cui, Mingyao and Wu, Zidong and Lu, Yu and Wei, Xiuhong and Dai, Linglong},
  journal={IEEE Communications Magazine}, 
  title={Near-Field {MIMO} Communications for {6G}: {F}undamentals, Challenges, Potentials, and Future Directions}, 
  year={2023},
  volume={61},
  number={1},
  pages={40-46},
  month = {January},
  }

  @article{sen2020teranova,
  title={The TeraNova platform: An integrated testbed for ultra-broadband wireless communications at true Terahertz frequencies},
  author={Sen, Priyangshu and Pados, Dimitris A and Batalama, Stella N and Einarsson, Erik and Bird, Jonathan P and Jornet, Josep M},
  journal={Computer Networks},
  volume={179},
  pages={107370},
  year={2020},
  publisher={Elsevier}
}

  @article{cui2022near,
  title={Near-field communications for 6G: Fundamentals, challenges, potentials, and future directions},
  author={Cui, Mingyao and Wu, Zidong and Lu, Yu and Wei, Xiuhong and Dai, Linglong},
  journal={IEEE Communications Magazine},
  year={2022},
  publisher={IEEE}
}
  
  @ARTICLE{combat_distance_chong,
  author={Akyildiz, Ian F. and Han, Chong and Nie, Shuai},
  journal={IEEE Communications Magazine}, 
  title={Combating the Distance Problem in the Millimeter Wave and Terahertz Frequency Bands}, 
  year={2018},
  volume={56},
  number={6},
  pages={102-108},
  month = {June},
  }

  @article{Schneider2012,
  doi = {10.1109/tthz.2011.2182118},
  url = {https://doi.org/10.1109/tthz.2011.2182118},
  year = {2012},
  month = mar,
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {2},
  number = {2},
  pages = {250--256},
  author = {Thomas Schneider and Andrzej Wiatrek and Stefan Preussler and Michael Grigat and Ralf-Peter Braun},
  title = {Link Budget Analysis for Terahertz Fixed Wireless Links},
  journal = {{IEEE} Transactions on Terahertz Science and Technology}
}

@article{sarieddeen2020next,
  title={Next generation terahertz communications: A rendezvous of sensing, imaging, and localization},
  author={Sarieddeen, Hadi and Saeed, Nasir and Al-Naffouri, Tareq Y and Alouini, Mohamed-Slim},
  journal={IEEE Communications Magazine},
  volume={58},
  number={5},
  pages={69--75},
  year={2020},
  publisher={IEEE}
}


@misc{vdi_antennas,
  title = {{VDI} Passive Devices},
  howpublished = {\url{https://www.vadiodes.com/en/products/straight-waveguides-tapers-horn-antenna-directional-couplers}},
  note = {Accessed: 2019-09-30}
}

@misc{miwave_antennas,
  title = {{Mi-Wave Antennas}},
  howpublished = {\url{https://www.miwv.com/millimeter-wave-products/antenna-products/}},
  note = {Accessed: 2019-09-30}
}

@article{fan2017development,
  title={Development of a high gain 325--500 GHz antenna using quasi-planar reflectors},
  author={Fan, Kuikui and Hao, Zhang-Cheng and Yuan, Quan and Hong, Wei},
  journal={IEEE Transactions on Antennas and Propagation},
  volume={65},
  number={7},
  pages={3384--3391},
  year={2017},
  publisher={IEEE}
}

@article{liaskos2019novel,
  title={A novel communication paradigm for high capacity and security via programmable indoor wireless environments in next generation wireless systems},
  author={Liaskos, Christos and Nie, Shuai and Tsioliaridou, Ageliki and Pitsillides, Andreas and Ioannidis, Sotiris and Akyildiz, Ian},
  journal={Ad Hoc Networks},
  volume={87},
  pages={1--16},
  year={2019},
  publisher={Elsevier}
}

@article{di2019smart,
  title={Smart radio environments empowered by reconfigurable {AI} meta-surfaces: An idea whose time has come},
  author={Di Renzo, Marco and others},
  journal={EURASIP J. on Wireless Commun. and Netw.},
  volume={2019},
  number={1},
  pages={1--20},
  year={2019},
  month={May},
}

@ARTICLE{llombart2011novel,
author={N. {Llombart} and G. {Chattopadhyay} and A. {Skalare} and I. {Mehdi}}, 
journal={IEEE Transactions on Antennas and Propagation}, 
title={Novel Terahertz Antenna Based on a Silicon Lens Fed by a Leaky Wave Enhanced Waveguide}, 
year={2011}, 
volume={59}, 
number={6}, 
pages={2160-2168}, 
keywords={antenna feeds;antenna radiation patterns;leaky wave antennas;lens antennas;silicon;submillimetre wave antennas;waveguide antennas;terahertz antenna;silicon lens;integrated arrays;hemispherical lens antenna;leaky wave waveguide feed;Schottky diodes;TE/TM leaky wave modes;resonant cavity;waveguide opening ground plane;f-number;off axis distortions;coating layer fabrication;reflection coefficient;phase center;off-axis displacement tolerance;far field radiation patterns;frequency 545 GHz;Lenses;Feeds;Cavity resonators;Silicon;Dielectrics;Optical waveguides;Iris;Leaky wave antennas;lenses;submillimeter wave technology}, 
doi={10.1109/TAP.2011.2143663}, 
ISSN={}, 
month={June},
}

@inproceedings{alqaraghuli2021performance,
  title={Performance analysis of a dual terahertz/ka band communication system for satellite mega-constellations},
  author={Alqaraghuli, Ali J and Abdellatif, Hussam and Jornet, Josep M},
  booktitle={2021 IEEE 22nd International Symposium on a World of Wireless, Mobile and Multimedia Networks (WoWMoM)},
  pages={316--322},
  year={2021},
  organization={IEEE}
}

@ARTICLE{Song2011,
author={H. {Song} and T. {Nagatsuma}},
journal={IEEE Transactions on Terahertz Science and Technology},
title={Present and Future of Terahertz Communications},
year={2011},
volume={1},
number={1},
pages={256-263},
keywords={modulation;radiocommunication;signal processing;telecommunication traffic;wireless channels;terahertz communications;multimedia services;mobile traffic;ultrafast wireless communications;advanced modulation;signal processing;microwave frequency;terahertz-wave technology;frequency 275 GHz to 3000 GHz;Wireless communication;Receivers;Modulation;Bandwidth;Transmitters;Attenuation;Power generation;Future wireless communications;terahertz communications;THz-waves},
doi={10.1109/TTHZ.2011.2159552},
ISSN={},
month={Sep.},}

@article{ma2018security,
  title={Security and eavesdropping in terahertz wireless links},
  author={Ma, Jianjun and Shrestha, Rabi and Adelberg, Jacob and Yeh, Chia-Yi and Hossain, Zahed and Knightly, Edward and Jornet, Josep Miquel and Mittleman, Daniel M},
  journal={Nature},
  volume={563},
  number={7729},
  pages={89--93},
  year={2018},
  publisher={Nature Publishing Group UK London}
}


@article{lu2021review,
  title={A review on applications of integrated terahertz systems},
  author={Lu, Xuyang and Venkatesh, Suresh and Saeidi, Hooman},
  journal={China Communications},
  volume={18},
  number={5},
  pages={175--201},
  year={2021},
  publisher={IEEE}
}

@article{akyildiz2022terahertz,
  title={Terahertz band communication: {An} old problem revisited and research directions for the next decade},
  author={Akyildiz, Ian F and others},
  journal={IEEE Trans. on Commun.},
  volume={70},
  number={6},
  pages={4250--4285},
  year={2022},
  month={June},
}

@article{sun2020implantable,
  title={Implantable, degradable, therapeutic terahertz metamaterial devices},
  author={Sun, Long and Zhou, Zhitao and Zhong, Junjie and Shi, Zhifeng and Mao, Ying and Li, Hua and Cao, Juncheng and Tao, Tiger H},
  journal={Small},
  volume={16},
  number={17},
  pages={2000294},
  year={2020},
  publisher={Wiley Online Library}
}

@article{chen2021terahertz,
  title={Terahertz wireless communications for 2030 and beyond: A cutting-edge frontier},
  author={Chen, Zhi and Han, Chong and Wu, Yongzhi and Li, Lingxiang and Huang, Chongwen and Zhang, Zhaoyang and Wang, Guangjian and Tong, Wen},
  journal={IEEE Communications Magazine},
  volume={59},
  number={11},
  pages={66--72},
  year={2021},
  publisher={IEEE}
}

@article{shiu2011physical,
  title={Physical layer security in wireless networks: A tutorial},
  author={Shiu, Yi-Sheng and Chang, Shih Yu and Wu, Hsiao-Chun and Huang, Scott C-H and Chen, Hsiao-Hwa},
  journal={IEEE wireless Communications},
  volume={18},
  number={2},
  pages={66--74},
  year={2011},
  publisher={IEEE}
}

@book{balanis2016antenna,
  title={Antenna theory: analysis and design},
  author={Balanis, Constantine A},
  year={2016},
  publisher={John Wiley \& Sons}
}

@article{petrov4mobile,
  title={Mobile Near-field Terahertz Communications for {6G} and {7G} Networks: {R}esearch Challenges},
  author={Petrov, Vitaly and Bodet, Duschia and Singh, Arjun},
  journal={Frontiers in Communications and Networks},
  volume={4},
  pages={6},
  year = {2023},
  publisher={Frontiers}
}

@inproceedings{singh2022wavefront,
  title={Wavefront Engineering at Terahertz Frequencies Through Intelligent Reflecting Surfaces},
  author={Singh, Arjun and Alqaraghuli, Ali J and Jornet, Josep M},
  booktitle={Proc. of the 23rd IEEE International Workshop on Signal Processing Advances in Wireless Communication (IEEE SPAWC)},
  pages={1--5},
  year={2022},
}

@article{ahmad2005synthetic,
  title={Synthetic aperture beamformer for imaging through a dielectric wall},
  author={Ahmad, Fauzia and Amin, Moeness G and Kassam, Saleem A},
  journal={IEEE transactions on aerospace and electronic systems},
  volume={41},
  number={1},
  pages={271--283},
  year={2005},
  publisher={IEEE}
}

@article{rappaport2019wireless,
  title={Wireless Communications and Applications Above 100 GHz: Opportunities and Challenges for 6G and Beyond},
  author={Rappaport, Theodore S and Xing, Yunchou and Kanhere, Ojas and Ju, Shihao and Madanayake, Arjuna and Mandal, Soumyajit and Alkhateeb, Ahmed and Trichopoulos, Georgios C},
  journal={IEEE Access},
  volume={7},
  pages={78729--78757},
  year={2019},
  publisher={IEEE}
}

@article{Llombart2022,
  doi = {10.1109/tap.2022.3168724},
  url = {https://doi.org/10.1109/tap.2022.3168724},
  year = {2022},
  month = aug,
  publisher = {Institute of Electrical and Electronics Engineers ({IEEE})},
  volume = {70},
  number = {8},
  pages = {7073--7083},
  author = {Nuria Llombart and Shahab Oddin Dabironezare},
  title = {Feasibility Study of Quasi-Optical {MIMO} Antennas for Radiative Near-Field Links},
  journal = {{IEEE} Transactions on Antennas and Propagation}
}

@article{abadal2013graphene,
  title={Graphene-enabled wireless communication for massive multicore architectures},
  author={Abadal, Sergi and Alarc{\'o}n, Eduard and Cabellos-Aparicio, Albert and Lemme, Max C and Nemirovsky, Mario},
  journal={IEEE Communications Magazine},
  volume={51},
  number={11},
  pages={137--143},
  year={2013},
  publisher={IEEE}
}

@article{goodman2005introduction,
  added-at = {2015-04-24T17:23:29.000+0200},
  author = {Goodman, Joseph W},
  biburl = {https://www.bibsonomy.org/bibtex/29478b0f25c5c971e1eb30ae74f86b5a5/gyllion},
  interhash = {7b67446d0c7d19c43b9539c71dccbe5c},
  intrahash = {9478b0f25c5c971e1eb30ae74f86b5a5},
  journal = {Introduction to Fourier optics, 3rd ed., by JW Goodman. Englewood, CO: Roberts \& Co. Publishers, 2005},
  keywords = {fourier optics},
  timestamp = {2015-04-24T17:23:29.000+0200},
  title = {Introduction to Fourier optics},
  volume = 1,
  year = 2005
}

@article{nokia_white_paper,
  author={Nokia},
  journal={White paper}, 
  title={Nokia’s vision for the {6G} era}, 
  year={2022},
  month = {January},
}

@article{docomo_white_paper,
  author={DOCOMO},
  journal={White paper}, 
  title={{5G Evolution and 6G}}, 
  year={2023},
  month = {January},
}


@ARTICLE{6g_proceedings,
  author={Tataria, Harsh and Shafi, Mansoor and Molisch, Andreas F. and Dohler, Mischa and Sjöland, Henrik and Tufvesson, Fredrik},
  journal={Proceedings of the IEEE}, 
  title={{6G} Wireless Systems: {V}ision, Requirements, Challenges, Insights, and Opportunities}, 
  year={2021},
  volume={109},
  number={7},
  pages={1166-1199},
  month={July},
}

@ARTICLE{6g_nyu,
  author={Rappaport, Theodore S. and Xing, Yunchou and Kanhere, Ojas and Ju, Shihao and Madanayake, Arjuna and Mandal, Soumyajit and Alkhateeb, Ahmed and Trichopoulos, Georgios C.},
  journal={IEEE Access}, 
  title={Wireless Communications and Applications Above {100 GHz}: {O}pportunities and Challenges for {6G} and Beyond}, 
  year={2019},
  volume={7},
  pages={78729-78757},
  month={June},
  }


@ARTICLE{slow_mmwave,
  author={Federico Agnoletto and Pau Castells and Emanuel Kolta and Dennisa Nichiforov-Chuang},
  journal={{GSM} Alliance white paper}, 
  title={The economics of {mmWave 5G}. {A}n assessment of total cost  of ownership in the period to 2025}, 
  month={June},
  year={2021},
  }


  @ARTICLE{thz_survey_chong,
  author={Han, Chong and Wang, Yiqin and Li, Yuanbo and Chen, Yi and Abbasi, Naveed A. and Kürner, Thomas and F. Molisch, Andreas},
  journal={IEEE Communications Surveys \& Tutorials}, 
  title={Terahertz Wireless Channels: {A} Holistic Survey on Measurement, Modeling, and Analysis}, 
  year={2022},
  volume={24},
  number={3},
  pages={1670-1707},
  month={thirdquarter},
  }

@techreport{ieee_802_15_3d,
type = {Standard},
key = {IEEE 802.15.3d--2017},
year = {2017},
title = {{IEEE 802.15.3d--2017: IEEE standard for high data rate wireless multi-media networks Amendment 2: 100 Gb/s wireless switched point-to-point physical layer}},
institution = {Institute of Electrical and Electronics Engineers},
}

@ARTICLE{Wyner1975,
  author={Wyner, A. D.},
  journal={The Bell System Technical Journal}, 
  title={The wire-tap channel}, 
  year={1975},
  volume={54},
  number={8},
  pages={1355-1387},
  month={October},
  }

  @article{depasse1995huygens,
  title={Huygens--Fresnel principle in the near field},
  author={Depasse, F and Paesler, MA and Courjon, D and Vigoureux, JM},
  journal={Optics letters},
  volume={20},
  number={3},
  pages={234--236},
  year={1995},
  publisher={Optical Society of America}
}

@article{durnin1988comparison,
  title={Comparison of Bessel and Gaussian beams},
  author={Durnin, J and Miceli, JJ and Eberly, Joseph H},
  journal={Optics letters},
  volume={13},
  number={2},
  pages={79--80},
  year={1988},
  publisher={Optical Society of America}
}

@article{han2021hybrid,
  title={Hybrid beamforming for terahertz wireless communications: Challenges, architectures, and open problems},
  author={Han, Chong and Yan, Longfei and Yuan, Jinhong},
  journal={IEEE Wireless Commun.},
  volume={28},
  number={4},
  pages={198--204},
  year={2021},
  month={Aug.},
}

  @article{durnin1987exact,
  title={Exact solutions for nondiffracting beams. {I}. {T}he scalar theory},
  author={Durnin, J},
  journal={JOSA A},
  volume={4},
  number={4},
  pages={651--654},
  year={1987},
  month={April},
  publisher={Optical Society of America},
}

@article{allen1992orbital,
  title={Orbital angular momentum of light and the transformation of Laguerre-Gaussian laser modes},
  author={Allen, Les and Beijersbergen, Marco W and Spreeuw, RJC and Woerdman, JP},
  journal={Physical review A},
  volume={45},
  number={11},
  pages={8185},
  year={1992},
  publisher={APS}
}

@article{siviloglou2007observation,
  title={Observation of accelerating {A}iry beams},
  author={Siviloglou, GA and others},
  journal={Phys. Review Letters},
  volume={99},
  number={21},
  pages={213901},
  year={2007},
  month={Nov.},
}

  @inproceedings{lipps2021towards,
  title={Towards the sixth generation (6G) wireless systems: Thoughts on physical layer security},
  author={Lipps, Christoph and Baradie, Shaden and Noushinfar, Marjan and Herbst, Jan and Weinand, Andreas and Schotten, Hans Dieter},
  booktitle={Mobile Communication-Technologies and Applications; 25th ITG-Symposium},
  pages={1--6},
  year={2021},
  organization={VDE}
}

@article{lin2012cosine,
  title={Cosine-Gauss plasmon beam: {A} localized long-range nondiffracting surface wave},
  author={Lin, Jiao and Dellinger, Jean and Genevet, Patrice and Cluzel, Benoit and de Fornel, Frederique and Capasso, Federico},
  journal={Physical Review Letters},
  volume={109},
  number={9},
  pages={093904},
  year={2012},
  publisher={{APS}},
}

@ARTICLE{chong_phy_layer_sec,
  author={Gao, Weijun and Chen, Yi and Han, Chong and Chen, Zhi},
  journal={IEEE Transactions on Wireless Communications}, 
  title={Distance-Adaptive Absorption Peak Modulation {(DA-APM)} for Terahertz Covert Communications}, 
  year={2021},
  volume={20},
  number={3},
  pages={2064-2077},
  month={March},
  }


@inproceedings{thz_sec_lwas,
author = {Yeh, Chia-Yi and Ghasempour, Yasaman and Amarasinghe, Yasith and Mittleman, Daniel M. and Knightly, Edward W.},
title = {Security in Terahertz {WLANs} with Leaky Wave Antennas},
year = {2020},
isbn = {9781450380065},
publisher = {Association for Computing Machinery},
booktitle = {Proc. of the 13th ACM Conference on Security and Privacy in Wireless and Mobile Networks},
pages = {317–327},
numpages = {11},
location = {Linz, Austria},
series = {WiSec '20},
month = {July},
}

@inproceedings{sherif_metasurface_2023,
author = {Shaikhanov, Zhambyl and Badran, Sherif and Jornet, Josep M. and Mittleman, Daniel M. and Knightly, Edward W.},
title = {Remotely Positioned MetaSurface-Drone Attack},
year = {2023},
publisher = {Association for Computing Machinery},
booktitle = {Proceedings of the 24th International Workshop on Mobile Computing Systems and Applications},
pages = {110–116},
numpages = {7},
series = {HotMobile '23},
month = {February},
}

@ARTICLE{nature_jornet,
author={Ma, Jianjun and Shrestha, Rabi and Adelberg, Jacob and Yeh, Chia-Yi and Hossain, Zahed and Knightly, Edward and Jornet, Josep Miquel and Mittleman, Daniel M.},
journal={Nature},
title={{Security and eavesdropping in terahertz wireless links}},
year={2018},
volume={563},
number={7729},
pages={89--93},
month={October},
}


@ARTICLE{mmwave_5G,
  author={Xiao, Ming and Mumtaz, Shahid and Huang, Yongming and Dai, Linglong and Li, Yonghui and Matthaiou, Michail and Karagiannidis, George K. and Björnson, Emil and Yang, Kai and I, Chih-Lin and Ghosh, Amitabha},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Millimeter Wave Communications for Future Mobile Networks}, 
  year={2017},
  volume={35},
  number={9},
  pages={1909-1935},
  month={September},
  }


  @ARTICLE{thz_channel_e,
  author={Dovelos, Konstantinos and Matthaiou, Michail and Ngo, Hien Quoc and Bellalta, Boris},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Channel Estimation and Hybrid Combining for Wideband Terahertz Massive {MIMO} Systems}, 
  year={2021},
  volume={39},
  number={6},
  pages={1604-1620},
  month={June},
  }

  @inproceedings{singh2022bessel,
  title={Bessel Beams for 6G-A Performance Analysis},
  author={Singh, Arjun and Reddy, Innem VAK and Bodet, Duschia and Jornet, Josep M},
  booktitle={2022 56th Asilomar Conference on Signals, Systems, and Computers},
  pages={658--664},
  year={2022},
  organization={IEEE}
}

  @inproceedings{dovelos2021intelligent,
  title={Intelligent reflecting surfaces at terahertz bands: Channel modeling and analysis},
  author={Dovelos, Konstantinos and Assimonis, Stylianos D and Ngo, Hien Quoc and Bellalta, Boris and Matthaiou, Michail},
  booktitle={2021 IEEE International Conference on Communications Workshops (ICC Workshops)},
  pages={1--6},
  year={2021},
  organization={IEEE}
}

@inproceedings{dovelos2021electromagnetic,
  title={Electromagnetic Modeling of Holographic Intelligent Reflecting Surfaces at Terahertz Bands},
  author={Dovelos, Konstantinos and Assimonis, Stylianos D and Ngo, Hien Quoc and Bellalta, Boris and Matthaiou, Michail},
  booktitle={2021 55th Asilomar Conference on Signals, Systems, and Computers},
  pages={415--420},
  year={2021},
  organization={IEEE}
}


  @ARTICLE{thz_mimo_hadi,
  author={Sarieddeen, Hadi and Alouini, Mohamed-Slim and Al-Naffouri, Tareq Y.},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Terahertz-Band Ultra-Massive Spatial Modulation {MIMO}}, 
  year={2019},
  volume={37},
  number={9},
  pages={2040-2052},
  month={September},
  }

  @ARTICLE{hadi_proc_ieee,
  author={Sarieddeen, Hadi and Alouini, Mohamed-Slim and Al-Naffouri, Tareq Y.},
  journal={Proceedings of the IEEE}, 
  title={An Overview of Signal Processing Techniques for Terahertz Communications}, 
  year={2021},
  volume={109},
  number={10},
  pages={1628-1665},
  month={October},
  }

@article{priyangshu_nature_electronics,
	title = {Multi-kilometre and multi-gigabit-per-second sub-terahertz communications for wireless backhaul applications},
	volume = {6},
	number = {2},
	journal = {Nature Electronics},
	author = {Sen, Priyangshu and Siles, Jose V. and Thawdar, Ngwe and Jornet, Josep M.},
	month = {February},
	year = {2023},
	pages = {164--175},
}

@ARTICLE{sergi_nano,
  author={Lemic, Filip and Abadal, Sergi and Tavernier, Wouter and Stroobant, Pieter and Colle, Didier and Alarcón, Eduard and Marquez-Barja, Johann and Famaey, Jeroen},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Survey on Terahertz Nanocommunication and Networking: {A} Top-Down Perspective}, 
  year={2021},
  volume={39},
  number={6},
  pages={1506-1543},
  month={June},
  }

  @ARTICLE{phy_layer_security_wcm,
  author={Shiu, Yi-Sheng and Chang, Shih Yu and Wu, Hsiao-Chun and Huang, Scott C.-H. and Chen, Hsiao-Hwa},
  journal={IEEE Wireless Communications}, 
  title={Physical layer security in wireless networks: a tutorial}, 
  year={2011},
  volume={18},
  number={2},
  pages={66-74},
  }

@article{phy_layer_security_survey,
author = {H. Vincent Poor  and Rafael F. Schaefer },
title = {Wireless physical layer security},
journal = {Proceedings of the National Academy of Sciences},
volume = {114},
number = {1},
pages = {19-26},
year = {2017},
month = {January},
}

@INPROCEEDINGS{absolute_security,
  author={Cohen, Alejandro and D'Oliveira, Rafael G. L. and Yeh, Chia-Yi and Guerboukha, Hichem and Shrestha, Rabi and Fang, Zhaoji and Knightly, Edward and Médard, Muriel and Mittleman, Daniel M.},
  booktitle={Proc. of the IEEE Conference on Communications and Network Security (CNS)}, 
  title={Absolute Security in High-Frequency Wireless Links}, 
  year={2022},
  volume={},
  number={},
  pages={46-54},
  month = {October},
  }


  @INPROCEEDINGS{emil_2021_asilomar,
  author={Bjornson, Emil and Demir, Ozlem Tuğfe and Sanguinetti, Luca},
  booktitle={Proc. of the 55th Asilomar Conference on Signals, Systems, and Computers (ASILOMAR)}, 
  title={A Primer on Near-Field Beamforming for Arrays and Reconfigurable Intelligent Surfaces}, 
  year={2021},
  volume={},
  number={},
  pages={105-112},
  month = {November},
  }

  @article{sengupta2018terahertz,
  title={Terahertz integrated electronic and hybrid electronic--photonic systems},
  author={Sengupta, Kaushik and Nagatsuma, Tadao and Mittleman, Daniel M},
  journal={Nature Electronics},
  volume={1},
  number={12},
  pages={622},
  year={2018},
  publisher={Nature Publishing Group}
}

  @article{sen2023multi,
  title={Multi-kilometre and multi-gigabit-per-second sub-terahertz communications for wireless backhaul applications},
  author={Sen, Priyangshu and Siles, Jose V and Thawdar, Ngwe and Jornet, Josep M},
  journal={Nature Electronics},
  volume={6},
  number={2},
  pages={164--175},
  year={2023},
  publisher={Nature Publishing Group UK London}
}

  @inproceedings{sen2019experimental,
  title={Experimental demonstration of ultra-broadband wireless communications at true terahertz frequencies},
  author={Sen, Priyangshu and Jornet, Josep M},
  booktitle={2019 IEEE 20th International Workshop on Signal Processing Advances in Wireless Communications (SPAWC)},
  pages={1--5},
  year={2019},
  organization={IEEE}
}


@misc{elbir2023nearfield,
      title={Near-Field Terahertz Communications: {M}odel-Based and Model-Free Channel Estimation}, 
      author={Ahmet M. Elbir and Wei Shi and Anastasios K. Papazafeiropoulos and Pandelis Kourtessis and Symeon Chatzinotas},
      year={2023},
      month = {February},
      eprint={2302.04802},
      archivePrefix={arXiv},
      primaryClass={eess.SP}
}



@techreport{fellerintroduction,
  title={An introduction to probability theory and its applications},
  author={Feller, William},
  year={1991},
  institution={Wiley series in probability and mathematical statistics, 3rd edn.}
}

@ARTICLE{sec_encoding,
  author={Wu, Yongpeng and Khisti, Ashish and Xiao, Chengshan and Caire, Giuseppe and Wong, Kai-Kit and Gao, Xiqi},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={A Survey of Physical Layer Security Techniques for {5G} Wireless Networks and Challenges Ahead}, 
  year={2018},
  volume={36},
  number={4},
  pages={679-695},
  month={April},
  }

  @ARTICLE{heath_wcl,
  author={Deshpande, Nitish and Castellanos, Miguel R. and Khosravirad, Saeed R. and Du, Jinfeng and Viswanathan, Harish and Heath, Robert W.},
  journal={IEEE Wireless Communications Letters}, 
  title={A Wideband Generalization of the Near-Field Region for Extremely Large Phased-Arrays}, 
  year={2023},
  volume={12},
  number={3},
  pages={515-519},
  month = {March},
  }

  @article{piesiewicz2007short,
  title={Short-range ultra-broadband terahertz communications: Concepts and perspectives},
  author={Piesiewicz, Radoslaw and Kleine-Ostmann, Thomas and Krumbholz, Norman and Mittleman, Daniel and Koch, Martin and Schoebei, Joerg and Kurner, Thomas},
  journal={IEEE Antennas and Propagation Magazine},
  volume={49},
  number={6},
  pages={24--39},
  year={2007},
  publisher={IEEE}
}

@article{federici2010terahertz,
  title={Review of terahertz and subterahertz wireless communications},
  author={Federici, John and Moeller, Lothar},
  journal={Journal of Applied Physics},
  volume={107},
  number={11},
  pages={111101},
  year={2010},
  publisher={AIP Publishing}
}


@ARTICLE{nf_pisa,
  author={Nepa, Paolo and Buffi, Alice},
  journal={IEEE Antennas and Propagation Magazine}, 
  title={Near-Field-Focused Microwave Antennas: {N}ear-field shaping and implementation}, 
  year={2017},
  volume={59},
  number={3},
  pages={42-53},
  month={June},
  }

  @ARTICLE{nf_localization,
  author={Friedlander, Benjamin},
  journal={IEEE Transactions on Signal Processing}, 
  title={Localization of Signals in the Near-Field of an Antenna Array}, 
  year={2019},
  volume={67},
  number={15},
  pages={3885-3893},
  month={August},
  }

  @ARTICLE{emil_power,
  author={Björnson, Emil and Sanguinetti, Luca},
  journal={IEEE Open Journal of the Communications Society}, 
  title={Power Scaling Laws and Near-Field Behaviors of Massive {MIMO} and Intelligent Reflecting Surfaces}, 
  year={2020},
  volume={1},
  pages={1306-1324},
  month={September},
  }


@ARTICLE{nf_1960_1,
  author={Kay, A.},
  journal={IRE Transactions on Antennas and Propagation}, 
  title={Near-field gain of aperture antennas}, 
  year={1960},
  volume={8},
  number={6},
  pages={586-593},
  month={November},
  }

  @ARTICLE{nf_1960_2,
  author={Hansen, R.},
  journal={IEEE Transactions on Antennas and Propagation}, 
  title={Focal region characteristics of focused array antennas}, 
  year={1985},
  volume={33},
  number={12},
  pages={1328-1337},
  month={December},
  }

  @misc{chong_technical,
      title={{N2-SAGE}: {N}arrow-beam Near-field {SAGE} Algorithm for Channel Parameter Estimation in {mmWave} and {THz} Direction-scan Measurements}, 
      author={Yuanbo Li and Yiqin Wang and Yi Chen and Ziming Yu and Chong Han},
      year={2022},
      eprint={2212.11756},
      archivePrefix={arXiv},
      primaryClass={cs.IT},
      month={November},
}

@misc{chong_magazine_nf_ff,
      title={Cross Far- and Near-field Wireless Communications in Terahertz Ultra-large Antenna Array Systems}, 
      author={Chong Han and Yuhang Chen and Longfei Yan and Zhi Chen and Linglong Dai},
      year={2023},
      eprint={2301.03035},
      archivePrefix={arXiv},
      primaryClass={cs.IT},
      month={January},
}


@INPROCEEDINGS{chong_uav,
  author={Li, Yuanbo and Li, Ning and Han, Chong},
  booktitle={Proc. of the IEEE ICC}, 
  title={Ray-tracing Simulation and Hybrid Channel Modeling for Low-Terahertz {UAV} Communications}, 
  year={2021},
  volume={},
  number={},
  pages={1-6},
  month={June},
  }

  @ARTICLE{xr_thz,
  author={Chaccour, Christina and Soorki, Mehdi Naderi and Saad, Walid and Bennis, Mehdi and Popovski, Petar},
  journal={IEEE Internet of Things Journal}, 
  title={Can Terahertz Provide High-Rate Reliable Low-Latency Communications for Wireless {VR}?}, 
  year={2022},
  volume={9},
  number={12},
  pages={9712-9729},
  month={June},
  }

  @INPROCEEDINGS{kuerner_thor,
  author={Kürner, Thomas and Kawanishi, Tetsuya},
  booktitle={Proc. of the IRMMW-THz}, 
  title={Demonstrating 300 {GHz} Wireless Backhaul Links – The {ThoR} Approach}, 
  year={2022},
  volume={},
  number={},
  pages={1-1},
  month={August},
  }


@article{siviloglou2007observation,
  title={Observation of accelerating {A}iry beams},
  author={Siviloglou, GA and others},
  journal={Physics Review Letters},
  volume={99},
  number={21},
  pages={213901},
  year={2007},
  month={November},
}

@inproceedings{priyangshu_thz_weather,
author = {Sen, Priyangshu and Hall, Jacob and Polese, Michele and Petrov, Vitaly and Bodet, Duschia and Restuccia, Francesco and Melodia, Tommaso and Jornet, Josep M.},
title = {Terahertz Communications Can Work in Rain and Snow: {I}mpact of Adverse Weather Conditions on Channels at 140 {GHz}},
year = {2022},
isbn = {9781450395090},
booktitle = {Proc. of the ACM Workshop on Millimeter-Wave and Terahertz Networks and Sensing Systems at ACM MobiCom},
pages = {13–18},
numpages = {6},
location = {Sydney, NSW, Australia},
series = {mmNets '22}
}

  
